SPEC: Seeing People in the Wild with an Estimated Camera

Due to the lack of camera parameter information for in-the-wild images, existing 3D human pose and shape (HPS) estimation methods make several simplifying assumptions: weak-perspective projection, large constant focal length, and zero camera rotation. These assumptions often do not hold and we show, quantitatively and qualitatively, that they cause errors in the reconstructed 3D shape and pose. To address this, we introduce SPEC, the first in-the-wild 3D HPS method that estimates the perspective camera from a single image and employs this to reconstruct 3D human bodies more accurately. First, we train a neural network to estimate the field of view, camera pitch, and roll given an input image. We employ novel losses that improve the calibration accuracy over previous work. We then train a novel network that concatenates the camera calibration to the image features and uses these together to regress 3D body shape and pose. SPEC is more accurate than the prior art on the standard benchmark (3DPW) as well as two new datasets with more challenging camera views and varying focal lengths. Specifically, we create a new photorealistic synthetic dataset (SPEC-SYN) with ground truth 3D bodies and a novel in-the-wild dataset (SPEC-MTP) with calibration and high-quality reference bodies. Both qualitative and quantitative analysis confirm that knowing camera parameters during inference regresses better human bodies. Code and datasets are available for research purposes at https://spec.is.tue.mpg.de.

==> sections/4_exps_dont_edit.tex <==
\section{Experiments}
\label{experiments}
\oh{we could use an introductory sentence here. What experiments are we doing to answer which kind of questions.}
\subsection{Datasets}

\paragraph{Pano360 dataset.} Previous work~\cite{Hold-Geoffroy_2018_CVPR, zhu2020single}, uses the SUN360~\cite{xiao2012recognizing} dataset to train camera calibration networks, however the dataset is no longer available due to licensing issues. Therefore, we have curated a new dataset of equirectangular panorama images called Pano360. The Pano360 dataset consists of 35K panoramic images of which 34K are from Flickr and 1K rendered from photorealistic 3D scenes. Following previous work~\cite{Hold-Geoffroy_2018_CVPR, zhu2020single}, we randomly sample the camera parameters pitch, roll, yaw, and vertical field-of-view to generate 400K training and 15K validation images. We use these to train our \camcalib model. More details on the dataset  are provided in the \supmat
% \paragraph{Pano-360 dataset} We have curated a dataset of 360-degrees equirectangular panorama images to train camera calibration head of our network. Pano-360 has 34117 high resolution panoramic images. These images are obtained from Internet and synthetic 3D scenes. To train single image camera calibration model, we sample 12 viewpoints per panorama image. 
\paragraph{\agoracam.} Existing datasets are captured using limited variation. Hence, they are not suitable for testing and training. We created a photorealistic synthetic dataset inspired by AGORA~\cite{patel2021agora} to train and evaluate our model. The AGORA dataset has high-quality textured human 3D scans from different vendors and provides ground-truth SMPL(X) parameters for them. We place these scans in 5 different high-quality photorealistic 3D scenes. These 3D scenes are quite large \oh{handwavy} and we optimize for maximum coverage. We randomly sample camera viewpoints and focal lengths to add diversity. Camera pitch is sampled from a uniform distribution $\mathcal{U}(-30^{\circ}, 15^{\circ})$, roll is sampled from a normal distribution $\mathcal{N}(0^{\circ}, 2.8^{\circ})$, and camera field-of-view from $\mathcal{U}(70^{\circ}, 130^{\circ})$ to cover the cameras used in everyday life \eg digital cameras, smartphones. In total, we obtained 22191 images/71982 instances for training, 3783 images/12071 instances for validation.

\paragraph{Mimic-the-pose Cam (MTP-Cam)}. MTP-Cam is a new test set for human pose, shape, and camera estimation. Following the idea of the MTP dataset~\cite{}, we ask a person to mimic 10 different poses. While the person remains in the pose, a video is being recorded, showing the person from different viewpoints. The camera is held at chest height, overhead, and close to the ground, through which perspective effects are generated. In addition, we ask each person to calibrate their camera, following a detailed protocol. We use a standard calibration toolbox~\cite{rehder2016extending} and keypoint detector~\cite{cao2018openpose} to obtain focal length, $\focalx$ and $\focaly$, and estimate 2D joints $\gtjoints{2}$, respectively. We extend the SMPLify-XC method and use the ground truth calibrated camera to fit the SMPL-X model to each video. In total, we collect 60 videos of 6 subjects (4 male, 2 female) who together mimic 60 different poses. 

The SMPLify-XC method is a three-stage optimization routine, that fits the SMPL-X model to an image, showing a person who is mimicking the pose of a presented SMPL-X mesh (MTP image). The pose $\tilde{\theta}$ and contact $\tilde{C}$ of the presented mesh constrain the optimization. Here, we introduce SMPLify-XC Cam, a method for fitting SMPL-X pose $\theta$ and shape $\beta$, as well as camera pitch $\pitch$, roll $\roll$, yaw $\yaw$, and translation $\camtransl$ to a MTP video captured in mannequin style. We also use three optimization stages, where the SMPLify-XC Cam first stage objective is given by   
\begin{equation}
E(\beta, \pitch, \roll, \yaw, \camtransl) = \lambda_M E_M + \sum_{i=1}^{F} E_{J_i} \text{.}
\end{equation}
$E_M$ denotes the SMPLify-XC shape loss, that takes the ground truth height and weight of a person into account. 
\begin{equation}
    E_{J_i} = \Big|\Big| \omega_i \gamma \big( \Pi \big(\mathcal{M}(\beta, \theta), \camrot_i, K, \camtransl_i \big) - \gtjoints{2}_i \big) \Big|\Big|^{2}_{2}
\end{equation}
denotes the 2D re-projection error of a single frame $i$ with ground truth 2D joints $\gtjoints{2}_i$, and camera rotation $\camrot_i$ and translation $\camtransl_i$. $\omega_i$ and$\gamma$ are per joint confidence and weight, respectively. $F$ is the number of frames per video, extracted at one frame per second. In the second and third stage, we seek to optimize 
\begin{align}
\begin{split}
E(\theta, \pitch, \roll, \yaw, \camtransl) = & \lambda_{m_h}E_{m_h} + \lambda_{\tilde{\theta}} E_{\tilde{\theta}} + \lambda_{\tilde{C}} E_{\tilde{C}} \\
                                        & \lambda_{S} E_{S} + \sum_{i=1}^{F} E_{J_i} \text{.}
\end{split}
\end{align}

$E_{m_h}$, $E_{\tilde{\theta}}$, $E_\tilde{C}$, $E_{S}$ denote the hand and presented pose priors, the presented contact loss and the general contact loss as defined in \cite{}, respectively.

% To construct \agoracam, we purchased \lea{used? them, and the SMPL fit is from AGORA} \mkocabas{Response to Lea: I thought about citing AGORA here; but it may violate the double submission policy since AGORA is not released yet.} high-quality textured human 3D scans from Renderpeople\cite{}. We have 1119 scans for training and 259 for validation. We fit SMPL to these scans to obtain ground-truth pose and shape. We place these scans in 5 different high-quality photorealistic 3D scenes. These 3D scenes are quite large and we optimize for maximum coverage of them. 


\paragraph{Others} In addition to the above datasets, we use the 3DPW~\cite{vonMarcard2018_3dpw}, COCO~\cite{coco}, MPI-INF-3DHP~\cite{mpiiinf3dhp_mono-2017}, and Human3.6M~\cite{ionescu_h36m} datasets. COCO, MPI-INF-3DHP, and Human3.6M are used for training, while 3DPW, \agoracam, and MTP-Cam are used for evaluation. Since there is no 3D body and camera annotations for COCO, we use \camcalib to attain pseudo camera parameters and SMPLify-X-cam to obtain pseudo 3D human body annotations. SMPLify-X-cam fitting is initialized via EFT~\cite{joo2020eft} annotations.


\paragraph{Evaluation metrics.} Mean per joint position error \mpjpe, procrusted-aligned mean per joint position error \pampjpe, and per vertex error \pve are the most commonly used evaluation metrics in the literature. In the current literature, methods assume known camera extrinsics and then compute \mpjpe, \pve in camera coordinates. However, this evaluation does not really reflect the performance of the existing method in in-the-wild settings where camera types and viewpoints are quite diverse. Therefore we propose using a variant of \mpjpe and \pve without assuming known camera extrinsics and compute the joint error in world coordinates which we call these metrics as \wmpjpe and \wpve. More details regarding the difference of evaluation metrics are discussed in greater detail in \supmat.

% We use standard evaluation metrics used in human body regression literature \ie mean per joint position error (\mpjpe) and procrusted-aligned mean per joint position error (\pampjpe) in $mm$ to evaluate pose estimation accuracy. Per vertex error (\pve) is used to evaluate shape accuracy. When computing \wmpjpe, all existing methods assume known camera extrinsic parameters and evaluate results in camera space. But here, we assume the camera extrinsics are unknown and compute the \wmpjpe in world coordinates. To be fair to existing methods, we also evaluate \cmpjpe after applying estimated camera parameters to their predictions and report \cmpjpe with that. \mkocabas{should we report both MPJPE versions or only the latter one?} Details regarding the evaluation are discussed in greater detail in \supmat.

\subsection{Implementation Details}
\label{sec:implementation}

\paragraph{\camcalib.} We follow the implementation of Geoffroy \etal~\cite{Hold-Geoffroy_2018_CVPR}. We use ResNet-50 as the backbone and predict $\pitch$, $\roll$, and $\vfov$ using separate fully-connected layers. Each parameter has 256 bins. The model is trained with variable size images for 30 epochs. Pano360 dataset is used for training and evaluation.

\paragraph{SMPLify-X-cam.} We use the original implementation of SMPLify-X with some modifications. Instead of starting from a mean pose and shape, we initialize the optimization from a regressor output. \oh{which?}
%in a similar spirit to SPIN~\cite{SPIN:ICCV:2019} 
%\lea{I find SPIN is confusing here. SMPLify-X-cam has nothing to do with a regression method, except that it's initialized from a regressor output.}. 
%To obtain an initial body translation $\bodytransl$, we use the Eq.~\ref{eq:body_transl}. 
Both for the first and second stage of optimization, the Adam optimizer with a step size of $10^{-2}$ is utilized for 100 steps.

\paragraph{SPEC.} Similar to the original HMR~\cite{kanazawa_hmr}, we use a ResNet-50 as the backbone and fully-connected layers applied iteratively to regress SMPL parameters. The Adam optimizer with a learning rate of $5e-5$ is used. For training, for the first 150 epochs, we start training with COCO and \agoracam datasets, and then incorporate MPI-INF-3DHP and Human3.6M datasets. Total training takes 175 epochs, $\sim$4-5 days.

\subsection{Single image camera calibration results}

We demonstrate the performance of different camera calibration methods on the Pano360 evaluation set in Table~\ref{tab:camcalib}. We report the mean angular error for camera pitch $\pitch$, roll $\roll$, and vfov $\vfov$. ScaleNet is from Zhu \etal~\cite{zhu2020single}, we use their open sourced implementation to obtain the result on Pano360. ScaleNet uses KL loss for training. We investigate the effect of different loss function \ie KL-divergence, \softltwo, and \softbiasedltwo with \camcalib network. \softbiasedltwo performs the best in comparison to different loss functions.
% In Figure~\ref{fig:cam_calib_results}, we show the results of a CNN model trained to estimate perspective camera parameters.

% \subsection{CamCalib results}

\begin{table}[]
    \centering
    \resizebox{0.49\textwidth}{!}{
        \npdecimalsign{.}
        \nprounddigits{2}
        \begin{tabular}{l|r|r|r}
            \toprule
            \textbf{Methods} & \textbf{vfov $\vfov^{\circ}$} $\downarrow$ & \textbf{pitch $\pitch^{\circ}$} $\downarrow$ & \textbf{roll $\roll^{\circ}$} $\downarrow$ \\ \midrule
            ScaleNet & 5.68 & 2.61 & 1.41 \\ \midrule
            \camcalib (KL Loss) & 3.53 & 2.32 & 1.15 \\ %\midrule
            \camcalib (\softltwo) & 3.34 & 2.06 & 1.11 \\ %\midrule
            \camcalib (\softbiasedltwo) & \bf 3.24 & \bf 1.94 & \bf 1.02 \\
            \bottomrule
        \end{tabular} 
    }
    \caption{Results of different methods Pano360 camera calibration dataset. ScaleNet~\cite{zhu2020single} results are obtained using authors' implementation.}
    \label{tab:camcalib}
\end{table}

\subsection{\smplify results}

Table~\ref{tab:smplify_agora} and \ref{tab:smplify_3dpw} summarize the performance of \smplify in comparison to the baseline SMPLify-x methods. The same 2D keypoint detections from \cite{mmpose2020} are used for all the reported methods. We compare the default setting of SMPLify-X with $f=5000$, the SMPLify-X setting used by Kissos \etal~\cite{kissosECCVW2020} where $f=2200$, and the SMPLify-X setting which uses \camcalib estimated $K, \camrot$. We observe a consistent improvement in \wmpjpe and \wpve when $\camrot$ is used. This is due to correct global orientation reconstruction wrt. world coordinates. On \agoracam using $K$ improves the \pampjpe due to more accurate projective geometry. 3DPW is limited in terms of camera variety. It is captured with a single camera where $f=1962$. Even in this case, \smplify improves the results over the default setting and the \pampjpe result is on par with when $f=2200$ used. This is because $f=2200$ approximation is already close to the single focal length used in 3DPW dataset $f=1962$. As a reference, the average \camcalib focal length error is 360, 246 pixels on 3DPW and \agoracam datasets, respectively.

%For table~\ref{tab:agora_cam_op}, an off-the-shelf 2d keypoint detection method is used to fit SMPL. Ground-truth 2D keypoints are used to obtain results in table~\ref{tab:agora_cam_gt}.

\begin{table}[]
    \centering
    \resizebox{0.49\textwidth}{!}{
        \begin{tabular}{l|r|r|r}
        \toprule
        \textbf{Methods} & \textbf{\wmpjpe} & \textbf{\pampjpe} & \textbf{\wpve} \\ \midrule
        SMPLify-X (ground-truth $f$) & 138.5 & 67.6 & 151.5 \\ 
        \midrule
        SMPLify-X ($f=5000$) & 179.3 & 71.6 & 191.5 \\ 
        SMPLify-X ($f=2200$) & 164.2 & 70.1 & 176.9 \\ 
        \midrule
        SMPLify-X (\camcalib $K$) & 143.3 & \textbf{67.4} & 156.3 \\
        \smplify (\camcalib $K$ + $\camrot$) & \textbf{121.9} & 67.8 & \textbf{135.0} \\ 
        \bottomrule
        \end{tabular} 
    }
    \caption{Results of \smplify on \agoracam dataset.}
    \label{tab:smplify_agora}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/focal_length_sensitivity.pdf}
    \caption{Sensitivity of SMPLify-X to focal length perturbation on \agoracam dataset. Using \camcalib estimated $f$ yields better results. Body reconstruction accuracy is less sensitive to larger focal lengths. Therefore, we propose \softbiasedltwo loss.}
    \label{fig:f_sensitivity}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{SPEC results}

\paragraph{Comparison to the state-of-the-art} Table~\ref{tab:sota_agora} and \ref{tab:sota_3dpw} show the results of a recent state-of-the-art (SOTA) methods on the \agoracam and the 3DPW datasets, respectively. To compute the \wmpjpe, \pampjpe, and \wpve metrics for other methods, we use their open source implementations. We use the HMR~\cite{kanazawa_hmr} method as our baseline and train it with identical settings \ie training datasets and optimization parameters as SPEC. SPEC outperforms the SOTA methods on both the \agoracam and 3DPW datasets. It also outperforms the HMR method which is trained in identical settings for fair comparison. The improvements in \wmpjpe and \wpve are significant because of more accurate camera geometry information both during training and inference.

\begin{table}[]
    \centering
    \resizebox{0.49\textwidth}{!}{
        \begin{tabular}{l|r|r|r}
        \toprule
        \textbf{Methods} & \textbf{\wmpjpe} & \textbf{\pampjpe} & \textbf{\wpve} \\ 
        \midrule 
        GraphCMR~\cite{kolotouros2019cmr} & 180.8 & 71.6 & 195.9  \\
        SPIN~\cite{SPIN:ICCV:2019} & 178.9 & 72.5 & 194.8 \\
        % Pose2Mesh~\cite{Choi_2020_ECCV_Pose2Mesh} & & & & & \\
        PartialHumans~\cite{Rockwell2020} & 187.5 & 82.2 & 202.6 \\
        I2L-MeshNet~\cite{Moon_2020_ECCV_I2L-MeshNet} & 180.8 & 71.6 & 195.9  \\
        % CenterHMR~\cite{CenterHMR} & 185.5 & 70.3 & 197.4 \\
        % CRMH~\cite{jiang2020mpshape} & & & & & \\ 
        \midrule
        HMR$^{*}$~\cite{kanazawa_hmr} & 126.5 & 51.9 & 138.4 \\
        SPEC & \textbf{78.1} & \textbf{49.9} & \textbf{92.8} \\
        \bottomrule
        \end{tabular} 
    }
    \caption{Results of SOTA methods on \agoracam dataset. We use the implementations provided by authors to obtain results. HMR$^{*}$ denotes that we train HMR using the same data as SPEC to make a fair comparsion. $^{\dagger}$ we use the SMPL output of this method instead of non-parametric mesh to be able to report \wpve.}
    \label{tab:sota_agora}
\end{table}

\begin{table}[]
    \centering
    \resizebox{0.49\textwidth}{!}{
        \begin{tabular}{l|r|r|r}
        \toprule
        \textbf{Methods} & \textbf{\wmpjpe} & \textbf{\pampjpe} & \textbf{\wpve} \\ 
        \midrule 
        GraphCMR~\cite{kolotouros2019cmr} &  &  &   \\
        SPIN~\cite{SPIN:ICCV:2019} &  &  &  \\
        % Pose2Mesh~\cite{Choi_2020_ECCV_Pose2Mesh} & & & & & \\
        PartialHumans~\cite{Rockwell2020} &  &  &  \\
        I2L-MeshNet~\cite{Moon_2020_ECCV_I2L-MeshNet} &  &  &   \\
        % CenterHMR~\cite{CenterHMR} & 185.5 & 70.3 & 197.4 \\
        % CRMH~\cite{jiang2020mpshape} & & & & & \\ 
        \midrule
        HMR$^{*}$~\cite{kanazawa_hmr} &  &  &  \\
        SPEC &  &  &  \\
        \bottomrule
        \end{tabular} 
    }
    \caption{Results of SOTA methods on MTP-Cam dataset. We use the implementations provided by authors to obtain results. HMR$^{*}$ denotes that we train HMR using the same data as SPEC to make a fair comparsion. $^{\dagger}$ we use the SMPL output of this method instead of non-parametric mesh to be able to report \wpve.}
    \label{tab:sota_mtp}
\end{table}

\begin{table}[]
    \centering
    \resizebox{0.49\textwidth}{!}{
        \begin{tabular}{l|r|r|r}
        \toprule
        \textbf{Methods} & \textbf{\wmpjpe} & \textbf{\pampjpe} & \textbf{\wpve} \\ 
        \midrule 
        % GraphCMR~\cite{kolotouros2019cmr} & 198.324 & 197.182 & 79.779 & 215.141 & 227.888 \\
        GraphCMR~\cite{kolotouros2019cmr} & 137.8 & 69.1 & 158.4 \\
        SPIN~\cite{SPIN:ICCV:2019} & 122.2 & 59.0 & 140.9 \\
        Partial Humans~\cite{Rockwell2020} & 139.4 & 76.9 & 160.1 \\
        I2L-MeshNet$^{\dagger}$~\cite{Moon_2020_ECCV_I2L-MeshNet} & 133.3 & 60.0 & 154.5 \\
        % CenterHMR~\cite{CenterHMR} & 130.3 & 60.8 & 149.3 \\
        \midrule
        HMR$^{*}$~\cite{kanazawa_hmr} & 122.3 & 55.3 & 139.4 \\
        SPEC & \textbf{106.4} & \textbf{53.2} & \textbf{127.4} \\ 
        \bottomrule
        \end{tabular} 
    }
    \caption{Results of SOTA methods on 3DPW test set. We use the implementations provided by authors to obtain results. HMR$^{*}$ denotes that we train HMR using the same data as SPEC to make a fair comparsion. $^{\dagger}$ we use the SMPL output of this method instead of non-parametric mesh to be able to report \wpve.}
    \label{tab:sota_3dpw}
\end{table}


\paragraph{Ablation experiments} We ablate different components of the SPEC model to investigate their effects on the final performance. We use the same datasets and training configurations for all methods. We use HMR as our baseline. To obtain the $\predjoints{2}$, HMR uses the bounding-box as the camera center. Hence, we start by changing the camera center to the image center \ie $o_x=\imgwidth/2, o_y=\imgheight/2$ denoted as ``HMR + $c$". This ensures a better projective geometry than using the bounding-box center as the image center and already improves results. Next, we replace the fixed focal length  of 5000 with t he values estimated by \camcalib and denote this with ``HMR + $c$ + $f$". ``HMR + $c$ + $f$ + $\camrot$" denotes the setting where $\camrot$ instead of $I$ is used as camera rotation during projection. Finally, SPEC denotes the use of $c$, $f$, $\camrot$ during projection and as an input to the final stage of HMR predictions.


\begin{table}[]
    \centering
    \resizebox{0.49\textwidth}{!}{
        \begin{tabular}{l|r|r|r}
        \toprule
        \textbf{Methods} & \textbf{\wmpjpe} & \textbf{\pampjpe} & \textbf{\wpve} \\ 
        \midrule
        HMR & 122.6 & 65.9 & 139.327 \\
        HMR + $c$ & 117.1 & 64.0 & 134.1 \\
        HMR + $c$ + $f$ &  &  &  \\
        \midrule
        HMR + $c$ + $f$ + $\camrot$ &  &  &  \\
        SPEC & \textbf{100.6} & \textbf{62.0} & \textbf{122.6} \\
        % SPEC - cam cond. & & & \\ 
        \bottomrule
        % HMR + cam center + gt fl + gt rot & & & \\ \hline
        \end{tabular} 
    }
    \caption{Ablation experiments on 3DPW validation set. $c$: using the image center as camera center, $f$ using \camcalib estimated focal length, $\camrot$ using \camcalib estimated camera rotation.}
    \label{tab:hmr_3dpw}
\end{table}

\begin{table}[]
    \centering
    \resizebox{0.49\textwidth}{!}{
        \begin{tabular}{l|r|r|r}
        \toprule
        \textbf{Methods} & \textbf{\wmpjpe} & \textbf{\pampjpe} & \textbf{\wpve} \\ 
        \midrule
        HMR & 138.3 & 53.9 & 149.9 \\
        HMR + $c$ & 126.5 & 51.9 & 138.4 \\
        HMR + $c$ + $f$ &  &  &  \\
        \midrule
        HMR + $c$ + $f$ + $\camrot$ & & & \\ 
        SPEC & \textbf{78.1} & \textbf{49.9} &\textbf{92.8} \\
        \bottomrule
        % HMR + cam center + gt fl + gt rot & & & \\ \hline
        \end{tabular} 
    }
    \caption{Ablation experiments on \agoracam dataset. $c$: using the image center as camera center, $f$ using \camcalib estimated focal length, $\camrot$ using \camcalib estimated camera rotation.}
    \label{tab:hmr_agora}
\end{table}


\begin{figure}[t]
    \centering
    \begin{minipage}{.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mpjpe_per_cam_pitch.pdf}
        % \captionof{figure}{A figure}
        \label{fig:test1}
    \end{minipage}%
    
    \begin{minipage}{.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mpjpe_per_focal_length.pdf}
        % \captionof{figure}{A figure}
        \label{fig:test1}
    \end{minipage}%
    \caption{Breakdown of \wmpjpe per camera focal length and pitch range.}
    \label{fig:error_breakdown}
    % \vspace{-2ex}
\end{figure}{}

\subsection{Qualitative Results}
Figure~\ref{fig:qualitative} shows qualitative results.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/qualitative.pdf}
    \caption{Qualitative results.\mkocabas{Figure is not final yet. I am working on it.} }
    \label{fig:qualitative}
    % \vspace{-2ex}
\end{figure*}{}

==> tables/results_agora.tex <==
\begin{table}
    \centering
    \resizebox{0.47\textwidth}{!}{
        \begin{tabular}{l|r|r|r}
        \toprule
        \textbf{Methods} & \textbf{\wmpjpe} & \textbf{\pampjpe} & \textbf{\wpve} \\ 
        \midrule 
        GraphCMR~\cite{kolotouros2019cmr} & 198.3 / 197.2 & 71.6 & 215.1 / 227.9 \\
        SPIN~\cite{SPIN:ICCV:2019} & 178.9 / 172.7 & 72.5 & 194.8 / 200.9 \\
        % Pose2Mesh~\cite{Choi_2020_ECCV_Pose2Mesh} & & & & & \\
        PartialHumans~\cite{Rockwell2020} & 187.5 / 191.3 & 82.2 & 202.6 / 220.7 \\
        I2L-MeshNet$^{\dagger}$~\cite{Moon_2020_ECCV_I2L-MeshNet} & 180.8 / 173.2 & 71.6 & 195.9 / 203.2  \\
        % CenterHMR~\cite{CenterHMR} & 185.5 & 70.3 & 197.4 \\
        % CRMH~\cite{jiang2020mpshape} & & & & & \\ 
        \midrule
        HMR$^{*}$~\cite{kanazawa_hmr} & 132.7 / 100.0 & 50.7 & 144.2 / 111.5 \\
        \methodname & \textbf{79.1} /\textbf{79.1} & \textbf{49.8} & \textbf{94.0} / \textbf{94.0} \\
        \bottomrule
        \end{tabular} 
    }
    \caption{Results of SOTA methods on \agoracam. See Table~\ref{tab:sota_mtp} caption.
    }
    \vspace{-1ex}
    \label{tab:sota_agora}
\end{table}

==> tables/results_agora_ablation.tex <==
\begin{table}
    \centering
    \resizebox{0.47\textwidth}{!}{
        \begin{tabular}{l|r|r|r}
        \toprule
        \textbf{Methods} & \textbf{\wmpjpe} & \textbf{\pampjpe} & \textbf{\wpve} \\ 
        \midrule
        
        HMR$^{*}$ & 132.7 / 100.0 & 50.7 & 144.2 / 111.5\\
        HMR$^{*}$ + $c$ & 123.9 / 89.3 & 50.3 & 136.6 / 100.4 \\
        HMR$^{*}$ + $c$ + $f$ & 121.5 / 87.1 & 50.1 & 134.1 / 99.1 \\ 
        \midrule
        HMR$^{*}$ + $c$ + $f$ + $\camrot$ & 81.8 / 81.8 & 50.2 & 96.2 / 96.2 \\ 
        \methodname & \textbf{79.1} / \textbf{79.1} & \textbf{49.8} & \textbf{94.0} / \textbf{94.0} \\
        \bottomrule
        % HMR + cam center + gt fl + gt rot & & & \\ \hline
        \end{tabular} 
    }
    \caption{Ablation studies with \agoracam. $c$: using the image center as camera center, 
    % $f$: using \camcalib estimated focal length, $\camrot$: using \camcalib estimated camera rotation.
    $f$ and $\camrot$: using \camcalib estimated focal length and camera rotation, respectively.
    }
    \vspace{-3ex}
    \label{tab:hmr_agora}
\end{table}

==> tables/results_mtp.tex <==
\begin{table}
    \centering
    \resizebox{0.47\textwidth}{!}{
        \begin{tabular}{l|r|r|r}
        \toprule
        \textbf{Methods} & \textbf{\wmpjpe} & \textbf{\pampjpe} & \textbf{\wpve} \\ 
        \midrule 
        GraphCMR~\cite{kolotouros2019cmr} & 181.1 / 173.1 & 92.5 & 202.7 / 194.2 \\
        SPIN~\cite{SPIN:ICCV:2019} & 165.0 / 151.7	& 79.2 & 189.7 / 164.4 \\
        % Pose2Mesh~\cite{Choi_2020_ECCV_Pose2Mesh} & & & & & \\
        PartialHumans~\cite{Rockwell2020} & 167.3 / 168.4	& 97.0 & 187.3 / 187.4 \\
        I2L-MeshNet$^{\dagger}$~\cite{Moon_2020_ECCV_I2L-MeshNet} & 172.2 / 171.9 & 91.3 & 196.4	/ 196.2 \\
        % CenterHMR~\cite{CenterHMR} & 185.5 & 70.3 & 197.4 \\
        % CRMH~\cite{jiang2020mpshape} & & & & & \\ 
        \midrule
        HMR$^{*}$~\cite{kanazawa_hmr} & 155.1 / 140.2 & 70.9 & 173.1 / 157.2  \\
        \methodname & \textbf{133.3} / \textbf{133.3}  &  \textbf{70.6} & \textbf{153.4} / \textbf{153.4} \\
        \bottomrule
        \end{tabular} 
    }
    \caption{Results of SOTA methods on MTP-Cam dataset. 
    We use the implementations provided by the authors. 
    HMR$^{*}$ means that we train HMR using the same data as \methodname for fair comparison. $^{\dagger}$means we use the SMPL output of this method instead of the non-parametric mesh to be able to report \wpve. All numbers are in \emph{mm}.
    %We use the implementations provided by authors to obtain results. HMR$^{*}$ denotes that we train HMR using the same data as \methodname to make a fair comparsion. $^{\dagger}$ we use the SMPL output of this method instead of non-parametric mesh to be able to report \wpve.
    }
    \vspace{-1ex}
    \label{tab:sota_mtp}
\end{table}

==> tables/supmat_agora.tex <==
\begin{table}
    \centering
    \resizebox{0.47\textwidth}{!}{
        \begin{tabular}{l|r|r|r|r|r}
        \toprule
        \textbf{Methods} & \textbf{\mpjpe} & \textbf{\wmpjpe} & \textbf{\pampjpe} & \textbf{\wpve} & \textbf{\pve}\\ 
        \midrule 
        GraphCMR~\cite{kolotouros2019cmr} & 195.6 & 198.3 / 197.2 & 71.6 & 215.1 / 227.9 & 216.8 \\
        SPIN~\cite{SPIN:ICCV:2019} & 171.0 & 178.9 / 172.7 & 72.5 & 194.8 / 200.9 & 185.8 \\
        % Pose2Mesh~\cite{Choi_2020_ECCV_Pose2Mesh} & & & & & \\
        PartialHumans~\cite{Rockwell2020} & 189.8 & 187.5 / 191.3 & 82.2 & 202.6 / 220.7 & 209.0 \\
        I2L-MeshNet$^{\dagger}$~\cite{Moon_2020_ECCV_I2L-MeshNet} & 171.6 & 180.8 / 173.2 & 71.6 & 195.9 / 203.2 & 194.4 \\
        % CenterHMR~\cite{CenterHMR} & 185.5 & 70.3 & 197.4 \\
        % CRMH~\cite{jiang2020mpshape} & & & & & \\ 
        \midrule
        HMR$^{*}$~\cite{kanazawa_hmr} & 90.0 & 132.7 / 100.0 & 50.7 & 144.2 / 111.5 & 102.0 \\
        \methodname & \textbf{77.9} & \textbf{79.1} /\textbf{79.1} & \textbf{49.8} & \textbf{94.0} / \textbf{94.0} & \textbf{92.2} \\
        \bottomrule
        \end{tabular} 
    }
    \caption{Results of SOTA methods on \agoracam. See Table~\ref{tab:sota_mtp} caption.
    }
    \vspace{-1ex}
    \label{tab:sota_agora}
\end{table}

==> tables/supmat_mtp.tex <==
\begin{table}
    \centering
    \resizebox{0.47\textwidth}{!}{
        \begin{tabular}{l|r|r|r|r|r}
        \toprule
        \textbf{Methods} & \textbf{\mpjpe} & \textbf{\wmpjpe} & \textbf{\pampjpe} & \textbf{\wpve} & \textbf{\pve}\\ 
        \midrule 
        GraphCMR~\cite{kolotouros2019cmr} & 157.8 & 181.1 / 173.1 & 92.5 & 202.7 / 194.2 & 178.0 \\
        SPIN~\cite{SPIN:ICCV:2019} & 138.4 & 165.0 / 151.7	& 79.2 & 189.7 / 164.4 & 149.7\\
        % Pose2Mesh~\cite{Choi_2020_ECCV_Pose2Mesh} & & & & & \\
        PartialHumans~\cite{Rockwell2020} & 162.0 & 167.3 / 168.4	& 97.0 & 187.3 / 187.4 & 178.8 \\
        I2L-MeshNet$^{\dagger}$~\cite{Moon_2020_ECCV_I2L-MeshNet} & 161.9 & 172.2 / 171.9 & 91.3 & 196.4 / 196.2 & 184.4 \\
        % CenterHMR~\cite{CenterHMR} & 185.5 & 70.3 & 197.4 \\
        % CRMH~\cite{jiang2020mpshape} & & & & & \\ 
        \midrule
        HMR$^{*}$~\cite{kanazawa_hmr} & \textbf{120.8} & 155.1 / 140.2 & 70.9 & 173.1 / 157.2 & \textbf{136.2} \\
        \methodname & 125.1 & \textbf{133.3} / \textbf{133.3}  &  \textbf{70.6} & \textbf{153.4} / \textbf{153.4} & 147.6 \\
        \bottomrule
        \end{tabular} 
    }
    \caption{Results of SOTA methods on \mtpcam dataset. 
    We use the implementations provided by the authors to obtain results. 
    HMR$^{*}$ means that we train HMR using the same data as \methodname for fair comparison. $^{\dagger}$means we use the SMPL output of this method instead of the non-parametric mesh to be able to report \wpve. All numbers are in \emph{mm}.
    %We use the implementations provided by authors to obtain results. HMR$^{*}$ denotes that we train HMR using the same data as \methodname to make a fair comparsion. $^{\dagger}$ we use the SMPL output of this method instead of non-parametric mesh to be able to report \wpve.
    }
    \vspace{-1ex}
    \label{tab:sota_mtp}
\end{table}

==> tables/supmat_smplify_agora.tex <==
\begin{table}[]
    \centering
    \resizebox{0.48\textwidth}{!}{
        \begin{tabular}{l|r|r|r}
        \toprule
        \textbf{Methods} & \textbf{\wmpjpe} & \textbf{\pampjpe} & \textbf{\wpve} \\ \midrule
        SMPLify-X (ground-truth $f$) & 138.5 / 119.9 & 67.6 & 151.5 / 133.4 \\ 
        \midrule
        SMPLify-X \cite{SMPL-X:2019} ($f=5000$) & 179.3 / 159.8 & 71.6 & 191.5 / 191.0 \\ 
        SMPLify-X \cite{kissosECCVW2020} ($f=2200$) & 164.2 / 141.8 & 70.1 & 176.9 / 155.3 \\ 
        \midrule
        SMPLify-X (\camcalib $K$) & 143.3 / 122.2 & \textbf{67.4} & 156.3 / 135.8 \\
        \smplify (\camcalib $K$ + $\camrot$) & \textbf{121.9} / \textbf{121.9} & 67.8 & \textbf{135.0} / \textbf{135.0} \\ 
        \bottomrule
        \end{tabular} 
    }
    \caption{{\bf HPS optimization with an estimated camera.}  \smplify on the \agoracam dataset.}
    \label{tab:smplify_agora}
\end{table}
